Improved quantum circuits for elliptic curve discrete logarithms

We present improved quantum circuits for elliptic curve scalar multiplication, the most costly component in Shor's algorithm to compute discrete logarithms in elliptic curve groups. We optimize low-level components such as reversible integer and modular arithmetic through windowing techniques and more adaptive placement of uncomputing steps, and improve over previous quantum circuits for modular inversion by reformulating the binary Euclidean algorithm. Overall, we obtain an affine Weierstrass point addition circuit that has lower depth and uses fewer $T$ gates than previous circuits. While previous work mostly focuses on minimizing the total number of qubits, we present various trade-offs between different cost metrics including the number of qubits, circuit depth and $T$-gate count. Finally, we provide a full implementation of point addition in the Q# quantum programming language that allows unit tests and automatic quantum resource estimation for all components.

==> pebbling.tex <==
The elliptic curve group law in Shor's algorithm and its components are built from quantum circuits for various classical functions that operate on bit strings of varying length $n$. A quantum circuit $U_f$ that computes such a function $f:\{0,1\}^n\rightarrow \{0,1\}^n$ can have different characteristics. It is often desirable to have the circuit compute $f$ \emph{in-place}, which means it implements the action $U_f: \ket{x} \mapsto \ket{f(x)}$ on inputs $x\in \{0,1\}^n$.
If $U_f$ is built out of Clifford$+T$ gates, each gate is easy to invert; thus, an in-place circuit $U_f$ automatically yields an in-place circuit $U_f^\dagger$ that computes $f^{-1}$. As quantum circuits need to be reversible, an in-place circuit is not always possible, e.g. if $f$ is not injective. 

\iffullversion
As an example consider modular multiplication. Let $p$ be an integer modulus. The function $f: (x,y)\mapsto (x,xy\mod p)$ is injective for inputs $x,y \in \Z/p\Z$ that are co-prime to $p$. Its inverse is modular division. At present, the best circuits we know to compute modular division use some variant of the Euclidean algorithm. Thus, an in-place modular multiplication circuit would either be more expensive than the Euclidean algorithm or would provide a state-of-the-art circuit for modular division.
\fi

When an in-place circuit is not possible, $U_f$ needs to implement $f$ \emph{out-of-place} as $\ket{x}\ket{0}^n\mapsto\ket{x}\ket{f(x)}$. Some circuits might even require a number of \emph{auxiliary qubits}, such that $U_f$ has the action
\iffullversion
\begin{equation}
\ket{x}\ket{0}^n\ket{0}^m\xmapsto{U_f}\ket{x}\ket{f(x)}\ket{g(x)},
\end{equation}
\else
$\ket{x}\ket{0}^n\ket{0}^m\mapsto\ket{x}\ket{f(x)}\ket{g(x)}$,
\fi
where $g$ is some function of the input. %We call the qubits containing $\ket{g(x)}$ \emph{dirty ancilla\michael[]{Aren't dirty ancilla qubits qubits that were already dirty (in any state) before applying the circuit?}\sam[]{I don't know what the common usage is. If that's what ``dirty ancilla'' normally means, then we should pick another term to refer to his, if such a term does not already exist. ``Entangled ancilla'' would work.}\michael{I think the term is just "ancilla qubits" or "ancillae". That's exactly what they are, I think it is clear that they are entangled with the rest.}}. 
The auxiliary qubits are entangled with the input and output qubit registers, at the end of the computation, they have to be returned to their original state, i.e. $g$ has to be \emph{uncomputed}. If there is a circuit $U_g$ for $g$, we can apply $U_g^\dagger$ to clear the auxiliary qubits:
\begin{equation}
\ket{x}\ket{0}^n\ket{0}^m\xmapsto{U_f}\ket{x}\ket{f(x)}\ket{g(x)}\xmapsto{U_g^\dagger}\ket{x}\ket{f(x)}\ket{0}^m.
\end{equation}
If it is computationally too costly or difficult (relative to the scale of the entire algorithm) to compute $g(x)$ from either $x$ or from $x$ and $f(x)$, one can use a generic standard trick due to Bennett~\cite{bennett1973} to clean the auxiliary qubits for any function. By adding another register of $n$ qubits, the output $f(x)$ is simply ``copied'' to that register using CNOT gates. Then, the inverse $U_f^\dagger$ is applied:
\begin{align}
\ket{x}\ket{0}^n\ket{0}^m\ket{0}^n\xmapsto{U_f} &\ket{x}\ket{f(x)}\ket{g(x)}\ket{0}^n\\
\xmapsto{\mathrm{CNOT}} & \ket{x}\ket{f(x)}\ket{g(x)}\ket{f(x)}\\
\xmapsto{U_f^\dagger} & \ket{x}\ket{0}^n\ket{0}^m\ket{f(x)}.
\end{align}
Applying these CNOT gates is often cheap relative to $U_f$ since $U_f$ needs at least $n$ gates to produce $f(x)$, and the CNOT gates can be applied simultaneously. Thus, besides requiring more qubits, the cost of this trick is roughly double the cost of $U_f$.

Clearly, the $k$-fold application of out-of-place circuits on $n$-qubit registers requires $k$ additional registers. A circuit for the function $f=f_n\circ f_{n-1}\circ\cdots\circ f_1$ produces a state
\iffullversion
\begin{equation}
\ket{x}\ket{f_1(x)}\ket{f_2(f_1(x))}\cdots \ket{f_k\circ\cdots\circ f_1(x)}.
\end{equation}
\else
$\ket{x}\ket{f_1(x)}\ket{f_2(f_1(x))}\cdots \ket{f_k\circ\cdots\circ f_1(x)}$.
\fi
Its size can quickly exceed the available number of qubits, in which case intermediate results have to be uncomputed before proceeding with the computation. Doing so adds significantly to the circuit depth. The extreme case uses only $\lg k$ registers, but requires a depth of $k^{\lg 3}$ applications of the single $U_{f_i}$.

The problem of optimizing a quantum circuit for a given number of qubit registers can be tackled by classical pebbling strategies\michael[]{Mathias? Insert citation for pebbling.}, where functions are carefully uncomputed and recomputed as needed.  

\subsubsection{Controlled circuits.}
As larger circuits are composed from smaller ones, the entirety of a smaller circuit often needs to be controlled with a single qubit. This can be done simply by ``promoting'' each Clifford$+T$ gate in the smaller circuit into a controlled variant. While this is cheap and easy for Clifford gates (though CNOT gates will become expensive Toffoli gates), controlled-T or controlled-Toffoli gates are much more expensive. A controlled-Toffoli gate requires an auxiliary qubit\sam[]{as far as I know - is there some more clever construction?}. Thus, we wish to be more clever in controlling smaller circuits. 

A circuit using Bennett's trick can be controlled by simply changing the CNOT gates into CCNOT gates as shown in Figure~\ref{fig:controlBennett} \iffullversion\else in Appendix~\ref{app:controlBennett}\fi. For other circuits, we will design controlled versions as needed.

\iffullversion
\begin{figure}
    \centering
    \begin{subfigure}[b]{0.4\textwidth}
    \centering
    \input{quantum-circuits/Qpic/bennett-reduction}
    \caption{Quantum circuit for reversible out-of-place computation of $f$ using Bennett's trick.}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.4\textwidth}
    \centering
    \input{quantum-circuits/Qpic/bennett-control}
    \caption{Controlled version of the same circuit with controls only added to the CNOT gates.}
    \end{subfigure}
    \caption{Adding control via a control qubit $\ket{c}$ to an out-of-place circuit using Bennett's trick for reversible computation of a function $f$ with circuit $U_f$.}\label{fig:controlBennett}
\end{figure}
\fi




==> quantum-circuits/Qpic/ECC-signed-windowed <==
PREAMBLE \providecommand{\ket}[1]{\left\vert #1\right\rangle}
PREAMBLE \providecommand{\gtxt}[1]{\texttt{#1}}

DEPTHPAD 2

sign W \ket{i_0}
address W \ket{i}
x1 W \ket{x_1}
y1 W \ket{y_1}
m W \ket{\lambda=0}
t0 W breadth=20
t1 W
t2 W
t3 W
t4 W

bonus W

address / \ell
x1 / n
y1 / n
m / n

-sign +address

address G $\gtxt{In}_i$ t0 t1 G $[i]P$ width=20

t0 G \rotatebox{270}{\gtxt{neg}} width=12 breadth=20 -sign
x1 G $-$ t0 G $-$
y1 G $-$ t1 G $-$

address G $\gtxt{In}_i$ t0 t1 G $[i]P$ width=20
TOUCH
x1 y1  m t0 t1 t2 t3 t4 G \rotatebox{270}{\gtxt{div}} width=10
bonus G ? width=18
TOUCH
x1 y1  m t0 t1 t2 G \rotatebox{270}{\gtxt{mul}}	 width=10
bonus G ? width=18

TOUCH
bonus G ? width=18
address G:breadth=10 $\gtxt{In}_i$ t0 G:breadth=30 \rotatebox{270}{$\scriptstyle{3([i]P)_x}$} width=15 
x1 G $+$ t0 G $+$
TOUCH
bonus G ? width=20	
address G:breadth=10  $\gtxt{In}_i$ t0 G:breadth=30 \rotatebox{270}{$\scriptstyle{3([i]P)_x}$} width=15 
TOUCH
bonus G ? width=18
x1 G $-$ m t0 t1 t2 G \rotatebox{270}{\gtxt{squ}} 
TOUCH
bonus G ? width=18
x1 G:breadth=19 \rotatebox{270}{\gtxt{mul}} y1 G:breadth=9 $+$ m t0 t1 t2 G \rotatebox{270}{\gtxt{mul}}
TOUCH
bonus G ? width=18
x1 y1 m t0 t1 t2 t3 t4 G \rotatebox{270}{\gtxt{div}} width=10
TOUCH
bonus G ? width=24
address G $\gtxt{In}_i$ t0 t1 G $[i]P$ width=20





t0 G \rotatebox{270}{\gtxt{neg}} -sign width=12 breadth=20

y1 G $-$ t1 G $-$
x1 G $-$ t0 G $-$

address G $\gtxt{In}_i$ t0 t1 G $[i]P$ width=20

+address -sign 

x1 G $\gtxt{neg}$ width=20

==> quantum-circuits/Qpic/ECC-windowed <==
PREAMBLE \providecommand{\ket}[1]{\left\vert #1\right\rangle}
PREAMBLE \providecommand{\gtxt}[1]{\texttt{#1}}

address W \ket{i}
x1 W \ket{x_1}
y1 W \ket{y_1}
z W \ket{z=0}
m W \ket{\lambda=0}
t0 W
t1 W
t2 W
t3 W
t4 W

address / \ell
x1 / n
y1 / n
m / n

address G $\gtxt{In}_i$ z G $([i]P)_z$ t0 t1 G $[i]P$ width=30

x1 G $-$ t0 G $-$
y1 G $-$ t1 G $-$

address G $\gtxt{In}_i$ z G $([i]P)_z$ t0 t1 G $[i]P$ width=30

x1 y1 G \gtxt{div} m t0 t1 t2 t3 t4 G \gtxt{div} z width=30
x1 y1 G \gtxt{mul} m t0 t1 G \gtxt{mul} width=30

address G $\gtxt{In}_i$ t0 G $3([i]P)_x$ width=40
x1 G $+$ t0 G $+$
address G $\gtxt{In}_i$ t0 G $3([i]P)_x$ width=40


x1 G \gtxt{squ}$^{-}$ m t0 t1 G \gtxt{squ}$^{-}$ width=30
x1 y1 G \gtxt{mul}$^+$ m t0 t1 G \gtxt{mul}$^+$ width=30
x1 y1 G \gtxt{div} m t0 t1 t2 t3 t4 G \gtxt{div} z width=30

address G $\gtxt{In}_i$ z G $([i]P)_z$ t0 t1 G $[i]P$ width=30

x1 G $+$ t0 G $+$
y1 G $+$ t1 G $+$
x1 G \gtxt{neg} width=20 z 

address G $\gtxt{In}_i$ z G $([i]P)_z$ t0 t1 G $[i]P$ width=30


==> quantum-circuits/Qpic/QDLP-square <==
PREAMBLE \providecommand{\ket}[1]{\left\vert #1\right\rangle}
PREAMBLE \providecommand{\gtxt}[1]{\texttt{#1}}

x1 W \ket{x_1}
y1 W \ket{y_1}
ctrl W \ket{\gtxt{ctrl}}
t0 W \ket{t_0=0}
m W \ket{\lambda}

x1 / n
y1 / n
t0 / n
m / n

m t0 G:width=30 \gtxt{squ}
t0 G {-} x1 G {-} ctrl
x1 G:width=30 $+3x^2$ ctrl
m t0 G:width=30 \gtxt{squ}

==> quantum-circuits/Qpic/bennett-control <==
PREAMBLE \providecommand{\ket}[1]{\left\vert #1\right\rangle}


oput W \ket{0} 
f W \ket{0} 
g W \ket{0} 
x W \ket{x} 
ctrl W \ket{c}


oput / n
f / n
g / m

x f g G $U_f$
f ctrl +oput
x f g G $U_f^\dagger$



==> quantum-circuits/Qpic/bennett-reduction <==
PREAMBLE \providecommand{\ket}[1]{\left\vert #1\right\rangle}

oput W \ket{0}
f W \ket{0}
g W \ket{0}
x W \ket{x}


oput / n
f / n
g / m

x f g G $U_f$
f +oput
x f g G $U_f^\dagger$



==> quantum-circuits/Qpic/fanin <==
PREAMBLE \providecommand{\ket}[1]{\left\vert #1\right\rangle}


x1 W \ket{x_1}
x2 W \ket{x_2}
a2 W 
x3 W \ket{x_3}
x4 W \ket{x_4}
a4 W 
a5 W
x5 W \ket{x_5}
x6 W \ket{x_6}
a6 W
ctrl W 
y W \ket{y}

y / m

a2 IN 0
a4 IN 0
a6 IN 0
TOUCH
x1 x2 +a2
x3 x4 +a4
x5 x6 +a6
a5 IN 0
TOUCH
a2 a4 +a5
ctrl IN 0
a5 a6 +ctrl
y G $G$ ctrl
a5 a6 +ctrl
ctrl OUT 0
a2 a4 +a5

TOUCH
a5 OUT 0
x5 x6 +a6
x3 x4 +a4
x1 x2 +a2

a2 OUT 0
a4 OUT 0
a6 OUT 0

==> quantum-circuits/Qpic/fanout <==
PREAMBLE \providecommand{\ket}[1]{\left\vert #1\right\rangle}


x1 W \ket{x_1}
a1 W
x2 W \ket{x_2}
a2 W 
x3 W \ket{x_3}
a3 W 
x4 W \ket{x_4}
a4 W 
x5 W \ket{x_5}
a5 W 
x6 W \ket{x_6}
ctrl W \ket{\ctrl}

a1 IN 0
a2 IN 0
a3 IN 0
a4 IN 0
a5 IN 0

ctrl +a3
ctrl +a5
a3 +a2
ctrl +a4
a3 +a1

TOUCH

x6 G $G$ ctrl
x5 G $G$ a5
x4 G $G$ a4
x3 G $G$ a3
x2 G $G$ a2
x1 G $G$ a1

a3 +a1
ctrl +a4
a3 +a2
ctrl +a5
ctrl +a3

TOUCH

a1 OUT 0
a2 OUT 0
a3 OUT 0
a4 OUT 0
a5 OUT 0

==> quantum-circuits/Qpic/kaliski-context <==
PREAMBLE \providecommand{\ket}[1]{\left\vert #1\right\rangle}
PREAMBLE \providecommand{\gtxt}[1]{\texttt{#1}}

u W \ket{u_i} 
v W \ket{v_i} 
r W \ket{r_i} 
s W \ket{s_i} 
m W \ket{m} 
f W \ket{f}
k W \ket{k} 
output W \ket{[x^{-1}2^{k-n}]} 

u / n
v / n
r / n+1
s / n+1
m / 2n
k / {\log n}
output / n

k G . fill=none color=white height=0 width=0

k +f
v G {$=0$} width=20 +f; +f
k G Inc width=25 -f
output G $/2$ width=20 -f
u v s r m G {Inversion Round} width=80 f
	

==> quantum-circuits/Qpic/mont-affine-no-b <==
PREAMBLE \providecommand{\ket}[1]{\left\vert #1\right\rangle}
PREAMBLE \providecommand{\gtxt}[1]{\texttt{#1}}

x1 W \ket{x_1}
y1 W \ket{y_1}
ctrl W \ket{\gtxt{ctrl}}
m W \ket{\lambda=0}
t0 W
t1 W
t2 W
t3 W
t4 W

x1 / n
y1 / n
m / n

x1 G $-x_2$ width=30
y1 G $-y_2$ width=30 ctrl
x1 y1 G \gtxt{div} m G \gtxt{div} t0 t1 t2 t3 t4 G \gtxt{div} ctrl width=30
x1 y1 G \gtxt{mul} m G \gtxt{mul} t0 t1 G \gtxt{mul} width=30
x1 G $+3x_2+a$ width=40
x1 G $\gtxt{squ}^+$ m t0 t1 G \gtxt{squ}$^+$ width=30
x1 y1 m t0 t1 G \gtxt{mul} width=30
x1 G $-2x_2$ width=30
x1 y1 G \gtxt{div} m G \gtxt{div} t0 t1 t2 t3 t4 G \gtxt{div} ctrl width=30
x1 G \gtxt{neg} width=20 ctrl
y1 G $-y_2$ width=30
x1 G $-x_2$ width=30 ctrl

==> quantum-circuits/Qpic/projective <==
PREAMBLE \providecommand{\ket}[1]{\left\vert #1\right\rangle}
PREAMBLE \providecommand{\gtxt}[1]{\texttt{#1}}

pp W \ket{P_x} \ket{0}
pmq W \ket{(P - Q)_x} \ket{(P-Q)_x}
out1 W \ket{0} \ket{0}
out2 W \ket{0} \ket{0}
ppq W \ket{0} \ket{(P+Q)_x}
q W \ket{Q_x} \ket{Q_x}

pp / n
pmq / n
out1 / n
out2 / n
ppq / n
q / n

pp pmq out1 out2 G \rotatebox{270}{\gtxt{DiffAdd}$_A$} q G {} width=30 
+out1 
+out2
out1 LABEL {(P+Q)_X}
out2 LABEL {(P+Q)_Z}
out1 out2 ppq G \gtxt{Div} width=30
pp pmq out1 out2 G \rotatebox{270}{\gtxt{DiffAdd}$_A^\dagger$} q G {} width=30

pp G {} out1 out2 ppq q G \rotatebox{270}{\gtxt{DiffAdd}$_A$} width=30
out1 LABEL {P_X}
out2 LABEL {P_Z}
pp G \gtxt{Div}$^-$ out1 out2 G \gtxt{Div}$^-$ width=30
pp G {} out1 out2 ppq q G \rotatebox{270}{\gtxt{DiffAdd}$_A^\dagger$} width=30




==> quantum-circuits/presentation/ECC-div-expanded <==
PREAMBLE \providecommand{\ket}[1]{\left\vert #1\right\rangle}
PREAMBLE \providecommand{\gtxt}[1]{\texttt{#1}}

x1 W 0 0 \ket{x_1}
y1 W 0 0 \ket{y_1}
ctrl W 0 0 \ket{\gtxt{ctrl}}
t0 W 0 0 \ket{t_0=0}
m W 0 0 \ket{\lambda}
t1 W 
t2 W
t3 W
t4 W
t5 W

x1 END
y1 END
ctrl END
t0 END
m END
t1 END
t2 END
t3 END
t4 END
TOUCH

t5 G 0 width=30
t5 END
TOUCH

x1 START
y1 START
ctrl START
t0 START
m START

TOUCH

x1 / n
y1 / n
m / n

t1 IN 0
t2 IN 0
t3 IN 0
t4 IN 0
t5 IN 0

x1 G \gtxt{inv}$_A$ width=30 height=20 t1 t2 t3 t4 t5 G \gtxt{inv}$_A$ 

x1 +t0

x1 G \gtxt{inv}$_A^{-1}$ width=30 height=20 t1 t2 t3 t4 t5 G \gtxt{inv}$_A^{-1}$ 

t1 OUT 0
t2 OUT 0
t3 OUT 0
t4 OUT 0
t5 OUT 0

t1 IN 0
t2 IN 0

y1 G \gtxt{mul}$_A$ width=30 t0  G \gtxt{mul}$_A$ width=30 t1 t2 G \gtxt{mul}$_A$ width=30
ctrl t1 +t0
y1 G \gtxt{mul}$_A^{-1}$ width=30 t0  G \gtxt{mul}$_A^{-1}$ width=30 t1 t2 G \gtxt{mul}$_A^{-1}$ width=30

t1 OUT 0
t2 OUT 0
 TOUCH

t1 IN 0
t2 IN 0
t3 IN 0
t4 IN 0
t5 IN 0

x1 G \gtxt{inv}$_A$ width=30 height=20 t1 t2 t3 t4 t5 G \gtxt{inv}$_A$ 

x1 +t0

x1 G \gtxt{inv}$_A^{-1}$ width=30 height=20 t1 t2 t3 t4 t5 G \gtxt{inv}$_A^{-1}$ 

t1 OUT 0
t2 OUT 0
t3 OUT 0
t4 OUT 0
t5 OUT 0

==> quantum-circuits/presentation/and <==
PREAMBLE \providecommand{\ket}[1]{\left\vert #1\right\rangle}

x W \ket{x} \ket{x}
y W \ket{y} \ket{y}
z W \ket{0} \ket{x\wedge y}

x y z G \rotatebox{270}{AND}


==> quantum-circuits/presentation/toffoli <==
PREAMBLE \providecommand{\ket}[1]{\left\vert #1\right\rangle}

x W \ket{x} \ket{x}
y W \ket{y} \ket{y}
z W \ket{z} \ket{z\oplus x\wedge y}

x y z G \rotatebox{270}{Toffoli}


==> quantum-circuits/presentation/upgrades <==
PREAMBLE \providecommand{\ket}[1]{\left\vert #1\right\rangle}

x W 
xctrl W
y W
yctrl W


xctrl END
yctrl END
TOUCH

x G $X$
y G $Z$
x END
y END
x START
xctrl START
y START
yctrl START
xctrl +x
y G $H$
yctrl +y
y G $H$



==> quantum-circuits/presentation/upgrades2 <==
PREAMBLE \providecommand{\ket}[1]{\left\vert #1\right\rangle}

x W 
x1 W
xctrl W
y W
y1 W
y2 W
yanc W
yctrl W

yanc END
xctrl END
yctrl END
y anc W
TOUCH

x1 +x
y1 y2 +y
x END
y END
x1 END
y1 END
y2 END
x START
x1 START
xctrl START
y START
y1 START
y2 START
yctrl START
xctrl x1 +x
yanc START
yctrl y2 +yanc
yanc y1 +y
yctrl y2 +yanc




==> windowing.tex <==
In Shor's algorithm, we use $2n$ qubits as control qubits, half of which controls circuits that add $P$, $2P$, $4P$, etc., and the other half with control addition of $Q$, $2Q$, etc. The points are added to a single quantum register which we will call the ``accumulator''. This requires $2n$ adders. We instead use a windowing approach, analogous to ubiquitous classical pre-computation techniques and similar to the techniques used for RSA \cite{GE2019}. 

The chain of adders enables us to create a superposition of up to $2^k$ states with $k$ additions. For a windowing approach, we instead ``load'' a superposition of points $P,2P,3P,\cdots,2^\ell P$ into an ancilla register which we will call the ``cache'', where the coefficient of $P$ is given by the input qubits. We then add the cache to the accumulator. For elliptic curves, this requires us to switch from a circuit adding a classical point to a circuit adding two quantum points, but this has little effect on the cost.% The expensive operations in point addition are modular inversion and modular multiplication, which are done on fully quantum inputs in either case. 

Loading classically precomputed points is equivalent to a QRAM access, indexed by the control qubits in Shor's algorithm. We can simulate QRAM access to $N$ elements with sequential circuits containg $4N$ T-gates \cite{babbushetal2018}. If we load points $\style{O},P,\cdots, 2^{\ell}P$, this will cost $4\cdot 2^{\ell}$ $T$-gates, but save us $\ell-1$ point additions. If point addition costs $\mathsf{A}$ many $T$ gates, we would expect $\ell\approx \lg(\mathsf{A}/4)$ to be the optimal value, leading to a factor $\ell$ reduction in T-gate cost.

Using this windowing technique requires 2 extra registers to store the precomputed points. Naively, we would need to keep these points for the full addition, since we must use the components of the second point three times during point addition (see Figure \ref{fig:ECC_full}). This would increase the total width of the algorithm by 2 registers. 

However, we can fit the look-ups within the existing space. As Figure \ref{fig:ECC_full} shows, at every point where $x_2$ or $y_2$ are added, the circuit spare ancillas available. Thus, we can perform the QRAM look-up, add the point to the quantum register, then uncompute the quantum look-up to free the qubits for the expensive modular division step. This requires us to do 3 QRAM look-ups rather than just one, but uses no extra registers. This would lead to an optimal $\ell$ of approximately $\lg(\mathsf{A}/12)$; since this differs by only a constant factor from an out-of-place windowing, we only analyze the in-place method.

A minor issue with windowing is that we will need to add the identity point, which the circuit in Figure \ref{fig:ECC_full} will not do correctly. To account for this, we add an extra $z$ qubit, which is $\ket{0}$ for the identity point and $\ket{1}$ otherwise. We use this qubit to control all of the operations in the point addition. This means we do not need any other control on the point addition. 

\subsection{Signed addition}
We can save a factor of 2 in windowing by using an extra bit to control the sign of $P$. Since $-P=(-P_x,P_y)$, the extra bit only needs to control a cheap modular negation. This changes the indexing slightly. Our original windowed circuit took an address register $\ket{b}$ and an input register $\ket{R}$, and produced $\ket{[b]P+R}$. Using the top bit of $b$ as a sign has the effect of
\begin{equation}
\sum_{b\in \{0,1\}^\ell} \ket{b}\ket{R} \mapsto \sum_{b\in\{0,1\}^\ell}\ket{b}\ket{[b-2^{\ell-1}]P+R}.
\end{equation}
Thus, we get an offset in each round, but since the offset is constant, it has no effect on the final phase estimation.


\sam{Maybe we should delete the remainder of this section, and only use what I wrote above.}
We can save a factor of 2 in windowing by using an extra bit to control the sign of $P$. Since $-P=(-P_x,P_y)$, we can use the extra bit to control a negation of $P_x$. With windowed addition, we divide our $n$ bits into $n=k\ell$. We run $k$ rounds, using $\ell$-bit controls for look-ups. To use signed windowing, we will divide each $\ell$-bit address $b$ into $(b_0,b')$, where $b_0$ is a single bit. We start by flipping the bit $b_0$, then flipping every bit of $b'$, conditioned on the value of $b_0$. In the last round, we will load $(b'+1)P$ into memory, then use $b_0$ to control a sign flip of $P_x$. We then add that to the register. This has the effect of:
\begin{equation}
\sum_{b\in \{0,1\}^\ell} \ket{b_0,b'}\ket{R} \mapsto \sum_{b\in\{0,1\}^\ell}\ket{b_0,b'}\ket{[b-2^{\ell-1}]P+R}.
\end{equation}
A similar technique works for earlier rounds, where we use $P^{\ell j}$ instead of $P$ in round $j$.

As we noted earlier, the affine Weierstrass circuit cannot correctly add $P$ and $Q$ if $P+Q=-P$. If we start with $R=\style{O}$, then every round will contain a point in the superposition that will not correctly add with one of the points in the next round. We can avoid this by starting with $R=P$. This will only cause a problem in the last round, where the accumulator and cache both contain points of the form $\pm 2^{\ell/2} P$. All four combinations will not add properly. However, at this point in the computation, these represent 4 states out of a superposition of $2^{n}$ states, so we will simply ignore this as a minor fidelity loss.

There is also a minor indexing issue. Shor's algorithm uses an eigenvalue estimation technique which uses a register $\ket{b}$ to control $b$ applications of some unitary $U$. In our case, $U$ adds a point $P$ to a register, so we require our circuit to map $\ket{b}\ket{R}$ to $\ket{b}\ket{[b]P+R}$. However, adding $-P$ does not have this same property. Using the high bits of $b$ in each round to control the sign means that controlling on $\ket{b}$ will add $[b-2^{n/2}-2^{(n-\ell)/2}-\ldots]P$ to the register (where $b$ has $n$ bits). This is the same as applying $U^b$ to an initial point of $[-2^{n/2}-2^{(n-\ell)/2}-\ldots]P+R$, and the eigenvalue estimation will still work correctly in this case. Thus, signed windowing will still function correctly.




\begin{figure}
\resizebox{\textwidth}{!}{
\input{quantum-circuits/Qpic/ECC-windowed}
}
\caption{Windowed elliptic curve addition, with $i$ address qubits. $\mathsf{In}_i$ is the indexing half of the look-up gate, which writes the classical data shown into the output registers.}\label{fig:ECC-windowed}
\end{figure}
\subsection{Alternative precomputation techniques}
A common technique in elliptic curve arithmetic is a ``comb''. In the comb, we wish to multiply a point $P$ by a scalar $k$, so we divide $k$ into $k_1+2k_2+\cdots + 2^\ell k_\ell$ for some $\ell$, with the property that $k_j$ contains bits of $k$ in positions congruent to $j$ modulo $\ell$ (each $k_j$ looks like a comb of bits). We then precompute a table all multiples of $P$ by scalars of the form $b_0+b_12^\ell+b_2 2^{2\ell}\cdots$, with $b_i\in\{0,1\}$. The definition of $k_j$ means that $k_jP$ will be in this table for all $j$. This, we can compute $kP$ by using $k_j$ to look up elements of the table, adding them to a running total, and doubling the running total. 

The advantage of the comb technique is that it saves us precomputation. We only precompute one table, and it is useful for the entire computation. Unfortunately for the quantum case, the pre-computation is essentially free because it's entirely classical, but look-ups are expensive. The comb technique gives no advantage for the number of table look-ups, since we need to do a separate look-up for each index $k_j$. 

Further, efficient in-place point doubling is unlikely, since it implies efficient in-place point halving. Thus, doubling points in the comb would require some pebbling technique which would likely add significant depth or width costs.



